A Diffusive T-Matrix Unifying the Electric and Magnetic Polarizability Tensors in Conducting Layered Media

Electromagnetic induction is used to detect and classify buried and submerged objects, such as unexploded ordnance in soil and on the seabed. A small object is commonly described by its magnetic polarizability tensor (MPT), which is independent of its position and of the sensor. The MPT assumes that the surrounding medium does not conduct. In seawater at extremely low frequency, or in clay at kilohertz frequencies, this assumption fails at depths comparable to the skin depth. The object then also diverts the current induced in the medium, a galvanic response that the MPT omits. We describe the object instead by its transition matrix (T-matrix), which keeps the independence from position and sensor and includes both responses. It is computed once per medium and frequency from a single finite element problem, for any shape and materials. Its inductive block reduces to the MPT when the medium conducts weakly, and its galvanic block reduces to the electric polarizability tensor in the static limit. We test the model against full finite element solutions for a conducting box, non-magnetic and permeable, in a layered sea and in clay over bedrock. Two orders beyond the dipole, it is accurate to within 1.4% over two decades of frequency and for sizes up to 0.7 of the depth, whereas the error of the MPT carried into the conducting medium reaches 91%. Blocks coupling the two responses, contained in neither tensor, contribute up to 13%.

==> xr-main.tex <==
\makeatletter
\newlabel{M-sec:intro}{{I}{1}{Introduction}{section.1}{}}
\newlabel{M-fig:scene}{{1}{2}{Geometry and structure of the model. The object lies in the top layer of a horizontally layered medium. The transmitter's field reaches the object as the drive $\vd $, the object responds through the T-matrix $\Tens $, and the response reaches the sensor through the propagator $\Prop $. Its reflections at the surface and at the interfaces below return to the object through $\Ret $}{figure.1}{}}
\newlabel{M-sec:model}{{II}{2}{Problem and Structure of the Model}{section.2}{}}
\newlabel{M-eq:perturbation}{{1}{2}{Problem and Structure of the Model}{equation.1}{}}
\newlabel{M-sec:governing}{{\mbox  {II-A}}{2}{Governing Equations}{subsection.2.1}{}}
\newlabel{M-eq:eddy}{{2}{2}{Governing Equations}{equation.2}{}}
\newlabel{M-eq:air}{{3}{2}{Governing Equations}{equation.3}{}}
\newlabel{M-sec:scaling}{{\mbox  {II-B}}{2}{Scaling to the Unit Object}{subsection.2.2}{}}
\newlabel{M-eq:scaling}{{4}{2}{Scaling to the Unit Object}{equation.4}{}}
\newlabel{M-eq:scaledpair}{{5}{2}{Scaling to the Unit Object}{equation.5}{}}
\newlabel{M-eq:helmholtz}{{6}{2}{Scaling to the Unit Object}{equation.6}{}}
\newlabel{M-eq:groups}{{7}{3}{Scaling to the Unit Object}{equation.7}{}}
\newlabel{M-eq:contrasts}{{8}{3}{Scaling to the Unit Object}{equation.8}{}}
\newlabel{M-sec:structure}{{\mbox  {II-C}}{3}{Structure of the Model}{subsection.2.3}{}}
\newlabel{M-eq:shape}{{9}{3}{Structure of the Model}{equation.9}{}}
\newlabel{M-sec:tensor}{{III}{3}{The T-Matrix}{section.3}{}}
\newlabel{M-sec:sea}{{\mbox  {III-A}}{3}{Modes of the Host}{subsection.3.1}{}}
\newlabel{M-eq:MN}{{10}{3}{Modes of the Host}{equation.10}{}}
\newlabel{M-eq:closure}{{11}{3}{Modes of the Host}{equation.11}{}}
\newlabel{M-eq:TE}{{12}{3}{Modes of the Host}{equation.12}{}}
\newlabel{M-eq:TM}{{13}{3}{Modes of the Host}{equation.13}{}}
\newlabel{M-eq:Psi}{{14}{3}{Modes of the Host}{equation.14}{}}
\newlabel{M-eq:Phi}{{15}{3}{Modes of the Host}{equation.15}{}}
\newlabel{M-eq:ambient}{{16}{3}{Modes of the Host}{equation.16}{}}
\newlabel{M-eq:response}{{17}{3}{Modes of the Host}{equation.17}{}}
\newlabel{M-sec:object}{{\mbox  {III-B}}{4}{The Transmission Problem and the Excess Sources}{subsection.3.2}{}}
\newlabel{M-eq:curlcurl}{{18}{4}{The Transmission Problem and the Excess Sources}{equation.18}{}}
\newlabel{M-eq:pert}{{19}{4}{The Transmission Problem and the Excess Sources}{equation.19}{}}
\newlabel{M-eq:weak}{{20}{4}{The Transmission Problem and the Excess Sources}{equation.20}{}}
\newlabel{M-eq:densities}{{21}{4}{The Transmission Problem and the Excess Sources}{equation.21}{}}
\newlabel{M-eq:withsources}{{22}{4}{The Transmission Problem and the Excess Sources}{equation.22}{}}
\newlabel{M-sec:extract}{{\mbox  {III-C}}{4}{Extraction by Reciprocity}{subsection.3.3}{}}
\newlabel{M-eq:reciprocity}{{23}{4}{Extraction by Reciprocity}{equation.23}{}}
\newlabel{M-eq:master}{{24}{4}{Extraction by Reciprocity}{equation.24}{}}
\newlabel{M-eq:reaction}{{25}{4}{Extraction by Reciprocity}{equation.25}{}}
\newlabel{M-eq:tensor}{{26}{4}{Extraction by Reciprocity}{equation.26}{}}
\newlabel{M-eq:integrandTE}{{27}{5}{Extraction by Reciprocity}{equation.27}{}}
\newlabel{M-eq:integrandTM}{{28}{5}{Extraction by Reciprocity}{equation.28}{}}
\newlabel{M-eq:response1}{{29}{5}{Extraction by Reciprocity}{equation.29}{}}
\newlabel{M-eq:symmetry}{{30}{5}{Extraction by Reciprocity}{equation.30}{}}
\newlabel{M-sec:surface}{{IV}{5}{Propagation Through Layered Media}{section.4}{}}
\newlabel{M-sec:sommerfeld}{{\mbox  {IV-A}}{5}{Transmission Through the Layers}{subsection.4.1}{}}
\newlabel{M-eq:sommerfeld}{{31}{5}{Transmission Through the Layers}{equation.31}{}}
\newlabel{M-eq:fromscalars}{{32}{5}{Transmission Through the Layers}{equation.32}{}}
\newlabel{M-eq:Ufree}{{33}{5}{Transmission Through the Layers}{equation.33}{}}
\newlabel{M-eq:admittance}{{34}{5}{Transmission Through the Layers}{equation.34}{}}
\newlabel{M-eq:RT}{{35}{5}{Transmission Through the Layers}{equation.35}{}}
\newlabel{M-eq:recursion}{{36}{6}{Transmission Through the Layers}{equation.36}{}}
\newlabel{M-eq:layerfactor}{{37}{6}{Transmission Through the Layers}{equation.37}{}}
\newlabel{M-eq:transmittedsource}{{38}{6}{Transmission Through the Layers}{equation.38}{}}
\newlabel{M-eq:kernel}{{39}{6}{Transmission Through the Layers}{equation.39}{}}
\newlabel{M-sec:propagator}{{\mbox  {IV-B}}{6}{The Propagator and the Drive}{subsection.4.2}{}}
\newlabel{M-eq:Qpoly}{{40}{6}{The Propagator and the Drive}{equation.40}{}}
\newlabel{M-eq:Q}{{41}{6}{The Propagator and the Drive}{equation.41}{}}
\newlabel{M-eq:Qprime}{{42}{6}{The Propagator and the Drive}{equation.42}{}}
\newlabel{M-eq:propentries}{{43}{6}{The Propagator and the Drive}{equation.43}{}}
\newlabel{M-eq:drivereciprocity}{{44}{6}{The Propagator and the Drive}{equation.44}{}}
\newlabel{M-eq:drive1}{{45}{6}{The Propagator and the Drive}{equation.45}{}}
\newlabel{M-sec:return}{{\mbox  {IV-C}}{6}{The Reflection Matrix}{subsection.4.3}{}}
\newlabel{M-eq:return}{{46}{6}{The Reflection Matrix}{equation.46}{}}
\newlabel{M-eq:gGamma}{{47}{6}{The Reflection Matrix}{equation.47}{}}
\newlabel{M-eq:reflectedsource}{{48}{7}{The Reflection Matrix}{equation.48}{}}
\newlabel{M-eq:reflectedfield}{{49}{7}{The Reflection Matrix}{equation.49}{}}
\newlabel{M-eq:retentries}{{50}{7}{The Reflection Matrix}{equation.50}{}}
\newlabel{M-eq:ret1}{{51}{7}{The Reflection Matrix}{equation.51}{}}
\newlabel{M-sec:assembled}{{\mbox  {IV-D}}{7}{The Assembled Model}{subsection.4.4}{}}
\newlabel{M-sec:properties}{{V}{7}{Structure and Limits of the T-Matrix}{section.5}{}}
\newlabel{M-sec:classical}{{\mbox  {V-A}}{7}{The MPT and the Polarization Tensor as Limits}{subsection.5.1}{}}
\newlabel{M-eq:mpt}{{52}{7}{The MPT and the Polarization Tensor as Limits}{equation.52}{}}
\newlabel{M-eq:pst}{{53}{7}{The MPT and the Polarization Tensor as Limits}{equation.53}{}}
\newlabel{M-sec:cross}{{\mbox  {V-B}}{8}{The Cross Blocks}{subsection.5.2}{}}
\newlabel{M-sec:rangelaws}{{\mbox  {V-C}}{8}{Range Laws in the Near Field}{subsection.5.3}{}}
\newlabel{M-eq:rangelaw}{{54}{8}{Range Laws in the Near Field}{equation.54}{}}
\newlabel{M-eq:ratio}{{55}{8}{Range Laws in the Near Field}{equation.55}{}}
\newlabel{M-sec:reductions}{{\mbox  {V-D}}{8}{Reduction to the Buried and Free-Space Models}{subsection.5.4}{}}
\newlabel{M-eq:buried}{{56}{8}{Reduction to the Buried and Free-Space Models}{equation.56}{}}
\newlabel{M-eq:epsfactor}{{57}{8}{Reduction to the Buried and Free-Space Models}{equation.57}{}}
\newlabel{M-sec:numerics}{{VI}{8}{Numerical Experiments}{section.6}{}}
\newlabel{M-fig:erroreps}{{2(a)}{9}{Subfigure 2(a)}{subfigure.2.1}{}}
\newlabel{M-sub@fig:erroreps}{{((a))}{(a)}{Subfigure 2(a)\relax }{subfigure.2.1}{}}
\newlabel{M-fig:errornu}{{2(b)}{9}{Subfigure 2(b)}{subfigure.2.2}{}}
\newlabel{M-sub@fig:errornu}{{((b))}{(b)}{Subfigure 2(b)\relax }{subfigure.2.2}{}}
\newlabel{M-fig:errorsize}{{2(c)}{9}{Subfigure 2(c)}{subfigure.2.3}{}}
\newlabel{M-sub@fig:errorsize}{{((c))}{(c)}{Subfigure 2(c)\relax }{subfigure.2.3}{}}
\newlabel{M-fig:errorepsperm}{{2(d)}{9}{Subfigure 2(d)}{subfigure.2.4}{}}
\newlabel{M-sub@fig:errorepsperm}{{((d))}{(d)}{Subfigure 2(d)\relax }{subfigure.2.4}{}}
\newlabel{M-fig:errornuperm}{{2(e)}{9}{Subfigure 2(e)}{subfigure.2.5}{}}
\newlabel{M-sub@fig:errornuperm}{{((e))}{(e)}{Subfigure 2(e)\relax }{subfigure.2.5}{}}
\newlabel{M-fig:errorsizeperm}{{2(f)}{9}{Subfigure 2(f)}{subfigure.2.6}{}}
\newlabel{M-sub@fig:errorsizeperm}{{((f))}{(f)}{Subfigure 2(f)\relax }{subfigure.2.6}{}}
\newlabel{M-fig:errors}{{2}{9}{Relative field error over the sensor ring in the sea and on land, (a)--(c)~for the non-magnetic box and (d)--(f)~for the permeable box, swept from the base case $\eps =0.05$, $\nua =30$, $\alpha /D=0.3$. (a), (d)~Against $\eps $, from $0.005$ to $0.5$ by the frequency, with $\sigma _*$ scaled to hold $\nua $. (b), (e)~Against $\nua $, from $3$ to $300$ by $\sigma _*$. (c), (f)~Against $\alpha /D$, from $0.2$ to $0.7$ at the base frequency, so that $D/\dels $ is fixed and $\eps $ grows as $\alpha ^2$, from $0.022$ to $0.27$}{figure.2}{}}
\newlabel{M-tab:setup}{{I}{9}{Parameters of the numerical experiments}{table.1}{}}
\newlabel{M-sec:conclusion}{{VII}{10}{Conclusion}{section.7}{}}
\makeatother

